Challenging the Human-in-the-loop in Algorithmic Decision-making

We discuss the role of humans in algorithmic decision-making (ADM) for socially relevant problems from a technical and philosophical perspective. In particular, we illustrate tensions arising from diverse expectations, values, and constraints by and on the humans involved. To this end, we assume that a strategic decision-maker (SDM) introduces ADM to optimize strategic and societal goals while the algorithms' recommended actions are overseen by a practical decision-maker (PDM) - a specific human-in-the-loop - who makes the final decisions. While the PDM is typically assumed to be a corrective, it can counteract the realization of the SDM's desired goals and societal values not least because of a misalignment of these values and unmet information needs of the PDM. This has significant implications for the distribution of power between the stakeholders in ADM, their constraints, and information needs. In particular, we emphasize the overseeing PDM's role as a potential political and ethical decision maker, who acts expected to balance strategic, value-driven objectives and on-the-ground individual decisions and constraints. We demonstrate empirically, on a machine learning benchmark dataset, the significant impact an overseeing PDM's decisions can have even if the PDM is constrained to performing only a limited amount of actions differing from the algorithms' recommendations. To ensure that the SDM's intended values are realized, the PDM needs to be provided with appropriate information conveyed through tailored explanations and its role must be characterized clearly. Our findings emphasize the need for an in-depth discussion of the role and power of the PDM and challenge the often-taken view that just including a human-in-the-loop in ADM ensures the 'correct' and 'ethical' functioning of the system.

==> figs/framework-readable.tex <==

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figs/framework-readable.png}
    \caption{Framework}
    \label{fig:framework-human-readble}
\end{figure}


==> theory.tex <==
\section{Machine Learning / Statistical Considerations}
\label{sec:theory}




\subsection{Explanations}
\label{sec:explanations}

To support the stakeholder's understanding of the decision-making process and its effect, different parts of the sequential process can be explained, cf.\ the dashed boxes in Figure~\ref{fig:framework}.
It has been shown that explanations can foster trust in ADM, help to identify biases and support debugging of models.
Most common in the literature are explanations about parts $E_1$ and $E_2$ of the model, i.e., explaining the predictions of the model, e.g., in the case of COMPAS this would mean that it is only explained how the software computes recidivism scores, and explaining the decisions derived from a model.
There is a plethora of explanation methods therefore, e.g., LIME, SHAP values, \ldots \sebastian{Extend list, add citations}.
While understanding $E_1$ and $E_2$ is important, in particular for model development, it might be insufficient for our considered setting.
In particular, in our setting is also important to consider explanations about parts $E_3$ and $E_4$:
\begin{itemize}
    
    
    \item $E_3$: The explanation includes the HIL.
      This is crucial importance in our setting as the HIL can alter the realized values and thereby counteract the political decisions made.
      It is thus important to clearly explain the operation of the HIL and what constraints might be put on the actions of the HIL.
      Note that explaining the role of HIL is particularly challenging as in many cases it can consider confounding information (which commonly is assumed to be used to correct an algorithm's mistakes) but could also be used differently.
      We expand this discussion in Sections~\ref{sec:philosophy} and~\ref{sec:theory}.
      
    \item $E_4$: The explanation includes the anticipated change in society. 
      This explanation can provide a most complete picture of the effects of an algorithm but also includes additional aspects which are hard to explain (in some cases it might also simply not be possible), e.g., how employment rate in society will change which will in most cases depend on additional exogenous confounding factors.
\end{itemize}

Clearly, the explanations form a hierarchy, with $E_4$ being more informative than $E_3$, which itself is more informative than $E_2$ and $E_1$.
While explanation $E_4$ is clearly of critical importance for \emph{solving} the political decision-making problem, it is not the main focus of our paper but we rather focus on $E_3$ and study the role of the HIL in depths.


The central problem we address in this paper is whether and, if, to what extend explanations can support the people in making choices in line with their values.















































